Detecting Human-Object Contact in Images

Humans constantly contact objects to move and perform tasks. Thus, detecting human-object contact is important for building human-centered artificial intelligence. However, there exists no robust method to detect contact between the body and the scene from an image, and there exists no dataset to learn such a detector. We fill this gap with HOT ("Human-Object conTact"), a new dataset of human-object contacts for images. To build HOT, we use two data sources: (1) We use the PROX dataset of 3D human meshes moving in 3D scenes, and automatically annotate 2D image areas for contact via 3D mesh proximity and projection. (2) We use the V-COCO, HAKE and Watch-n-Patch datasets, and ask trained annotators to draw polygons for the 2D image areas where contact takes place. We also annotate the involved body part of the human body. We use our HOT dataset to train a new contact detector, which takes a single color image as input, and outputs 2D contact heatmaps as well as the body-part labels that are in contact. This is a new and challenging task that extends current foot-ground or hand-object contact detectors to the full generality of the whole body. The detector uses a part-attention branch to guide contact estimation through the context of the surrounding body parts and scene. We evaluate our detector extensively, and quantitative results show that our model outperforms baselines, and that all components contribute to better performance. Results on images from an online repository show reasonable detections and generalizability.

==> paper/06_conclusions.tex <==
\section{Conclusion}
\label{sec:conclusion}

We focus on human-object contact detection for images. 
To this end, we collect the \hot dataset and develop the \hot contact detector with human-part guided attention. 
Our detector outperforms baseline models and generalizes reasonably well for in-the-wild images. 
Experiments show empirically that human-part attention is critical for contact estimation. 
Our data and model go beyond existing work towards a general-purpose full-body contact detector. 
We believe that this new task, dataset and model fill a gap in the literature, and help the community for several applications. 

{\small
\qheading{Acknowledgments}
We thank Chun-Hao Paul Huang for his valuable help with the RICH data and the training code of BSTRO \cite{huang2022capturing}. 
We thank Lea M\"{u}ller, Mohamed Hassan, Muhammed Kocabas, Shashank Tripathi, and Hongwei Yi for the insightful discussions. 
We thank Benjamin Pellkofer for the IT support, and Nicole Overbaugh and Johanna Werminghausen for administrative help. 
This work was supported by the German Federal Ministry of Education and Research (BMBF): T{\"u}bingen AI Center, FKZ: 01IS18039B.}

{\small
\qheading{Disclosure / Conflict of Interest}
MJB has received research gift funds from Adobe, Intel, Nvidia, Meta/Facebook, and Amazon.  
MJB has financial interests in Amazon, Datagen Technologies, and Meshcapade GmbH.  
While MJB was a part-time employee of Amazon during a portion of this project, his research was performed solely at, and funded solely by, the Max Planck Society.}

\vspace{-0.5 em}
\noindent\rule{\linewidth}{1.5pt}
\vspace{-1.5 em}

